A Typing System for the Linear Lambda-Calculus in de Bruijn Notation

We introduce a typing system that is particularly well suited for typing the linear lambda-calculus in de Bruijn notation. This typing discipline, which is reminiscent of Hodas' and Miller's model of resource consumption, guarantees that any well-typed term is linear without the need for an occurrence check. We then establish the subject reduction property.

==> eptcsdata.tex <==
\providecommand{\firstpage}{71}
\providecommand{\publicationstatus}{V. de Paiva; T.A. de Lima (Eds.): 21st International Symposium\\ on Logical and Semantic Frameworks, with Applications (LSFA 2026)\\
EPTCS 449, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.449.5}{10.4204/EPTCS.449.5}}
\pdfoutput=1

